VenusRL: A Fully Disaggregated Agentic RL System with Priority Scheduling and Scalable Interaction

Agentic Reinforcement Learning (RL) trains LLM agents through multi-turn interactions with external tool environments. Its multi-turn nature exposes two system-level bottlenecks unaddressed by existing agentic RL frameworks. First, end-to-end training throughput is constrained by the slowest trajectories to complete, yet optimizing per-GPU utilization alone scatters rollout progress across many groups, delaying the completion of enough groups to unblock the next training step. Second, tool sandboxes are statically over-provisioned by their declared memory ceilings, leaving most physical memory stranded while replicating near-identical state across sandboxes launched from the same prompt. We present VenusRL, a fully disaggregated agentic RL system that addresses both bottlenecks. VenusRL's priority-aware action scheduler uses length-prediction heuristics to identify sample groups whose completion is most likely to unblock the next training step, and pushes them ahead of others across batch admission, KV Cache residency, and cross-worker request orchestration. VenusRL's environment resource manager combines a memory-aware admission threshold with a template-keyed page-sharing pool, packing more sandboxes per node while preserving strict memory isolation via write-protected page table entry aliasing and copy-on-write. Across representative agentic RL workloads, VenusRL achieves up to 4.24x end-to-end training speedup over state-of-the-art baselines and reduces environment cost by up to 89%.

==> textFiles/1Introduction.tex <==
\section{Introduction}


% %Reinforcement Learning(RL) has recently achieved remarkable successes in training several large language models(LLM). However, existing LLM applications have progressively extended from mere chatbots to autonomous agents capable of handling long-horizon real-world tasks. When addressing complex tasks, these agents must learn to interact with external environments and utilize tools to enhance their reasoning capabilities - an emerging paradigm referred to as agentic RL.


% %Recent research has evolved the environment interaction in agentic reinforcement learning from \textit{single-turn} setting to \textit{multi-turn}, where an agent continuously interacts with the external environment and learns through self-reflection. However, multi-turn interaction incurs one of the two major system challenges in agentic RL training: \textbf{How to address great GPU underutilization and inefficiency}? 



% Agentic Reinforcement Learning (Agentic RL) has emerged as an important paradigm, enabling Large Language Models (LLMs) to solve complex tasks through iterative interaction with external environments. 
% Unlike traditional static generation, Agentic RL introduces a dynamic \texttt{Reasoning $\leftrightarrow$ Tool-Call} workflow, alternating between generating reasoning traces and executing external tools.
% This process is characterized by three distinct attributes. 
% First, the interaction is multi-turn, where the sequential dependency between reasoning and tool execution creates intrinsic GPU idle periods that we term as \texttt{turn-level agentic bubbles}. 
% Second, the workload is multi-task, necessitating the simultaneous management of various types of environment instances.
% \zmh{Third, agent behavior exhibits tool convergence, although the environment instances' types are diverse, utilization gradually concentrates on a specific subset of them, with their invocation frequency increasing as training progresses.}

% \begin{figure}[t]
%     \includegraphics[width=0.9\linewidth]{Figure/plot/skewnessbubble.png}
%     \centering
%     \vspace{-0.5\baselineskip}
%     \caption[Caption for LOF]{\zmh{Two types of Skewness Bubble in RL}}
%     \label{skewness bubble}
%     \vspace{-1\baselineskip}
% \end{figure}


% According to the attributes of Agentic RL, we believe that an ideal Agentic RL framework must attain three high-level design goals:
% (1) extreme resource elasticity to strictly balance training costs with system efficiency, 
% (2) continuous computation saturation to mitigate the inefficiencies of turn-level agentic bubbles, 
% and (3) bounded algorithmic relaxation to ensure that throughput optimizations remain strictly subservient to model convergence quality.

% \zmh{However, existing systems fail to achieve the goals above.}
% Traditional RLHF frameworks (e.g., HybridFlow~\cite{Sheng_2025}, verl) rely on static, staged pipelines (Generation $\rightarrow$ Inference), lacking the flexibility to manage dynamic interaction bubbles or multi-task scaling. 
% On the other hand, asynchronous solutions (e.g., ROLL Flash~\cite{lu2025iirollflash}) attempt to mask latency but suffer from critical deficiencies. 
% First, they rely on static resource provisioning, ignoring the tool convergence pattern, which results in significant resource waste. 
% Second, their scheduling strategies are agnostic to workload characteristics that they fail to analyze the significant variance in tool-call durations across different multi-task environments and neglect the sequential dependencies inherent in multi-turn interactions. 
% Consequently, this blind filling of bubbles leads to severe blocking delays that exacerbate off-policy staleness, ultimately degrading model convergence.
% %这一句可以换成两个都不能解决agentic rl的问题


% To satisfy these objectives, a fundamental architectural shift is required %机遇存在于The chance lies in
% to decouple the environmental interaction substrate from the core algorithmic architecture. 
% Current frameworks rigidly treat environments as fixed, hard-coded objects, making them incapable of handling dynamic turn-level agentic bubbles or multi-task scaling. 
% Our core insight is to abstract resource management into a unified lower level while centralizing interaction dispatching at a higher level. 
% This separation endows the system with the elasticity to mask physical constraints and the global awareness to inject computation into idle bubbles. 
% Guided by this philosophy, we propose \X, a general and efficient I/O layer designed to mediate these decoupled interactions.

% However, realizing this decoupled design faces two key challenges.
% First, achieving efficient elastic scaling is constrained by the significant setup latency of environment instances. 
% If scaling speed fails to keep up with demand, it creates performance bottlenecks where GPUs are forced to idle while waiting for environments. 
% Conversely, if scaling is too aggressive or exceeds actual needs, it leads to substantial resource waste and inflated training costs. 
% Second, there is an intrinsic conflict between handling bubble uncertainty and maintaining algorithmic convergence. 
% The extreme variance in multi-task tool-call durations creates highly unpredictable turn-level agentic bubbles. 
% Naively filling these irregular gaps to maximize throughput risks exacerbating off-policy staleness, creating a paradox where higher GPU utilization degrades model quality and fails to translate into faster training.

% \X proposes two core system innovations to cope with these two challenges.
% First, to address the challenge of resource elasticity, 
% % a naive approach relies on Reactive Scaling, which triggers allocation only upon immediate demand. 
% % However, this inherently fails due to significant environment setup latencies, leading to unavoidable under-provisioning and GPU starvation. 
% \X employs predictive scaling, which forecasts tool usage growth to proactively initiate environment creation, effectively overlapping setup time with active training to ensure resources are ready precisely when needed.
% Second, to resolve the conflict between throughput and convergence, 
% % a naive solution employs Aggressive Overlap, blindly inserting new tasks into idle slots. 
% % However, this coarse-grained scheduling distorts the execution order of trajectories, exacerbating off-policy staleness and degrading model quality. 
% \X introduces a speculative rollout with preemptive interruption. 
% By injecting speculative inference tasks into turn-level agentic bubbles and immediately terminating them upon tool completion, we ensure continuous GPU saturation while rigorously preserving the on-policy fidelity of the primary trajectory.

% \zmh{lack the implementation and evaluations}


% In summary, our contributions are as follows:
% \begin{itemize}
%     \item We propose AIO, the first IO layer to systematically decouple environment management from the training framework, enabling global awareness and preemption.
%     \item We introduce Predictive Scaling and Speculative Rollout with Interruption, solving the intrinsic conflict between system throughput and algorithmic convergence.
%     \item Extensive experiments demonstrate that AIO achieves superior throughput and convergence speed compared to state-of-the-art baselines.
% \end{itemize}

% %Concretely, skewness bubble serves as one of the mainstream bubbles in RL, originating from skewed distribution of response length within one batch. Making the problem even worse, as illustrated in Figure 1, the uncertainty of turn numbers and imbalance interaction time of agentic RL incur completely unpredictable output lengths, which means a more serious long-tail effect. Recent researchers have advocated for a disaggregated reinforcement learning framework, employing a decoupled and fully asynchronous approach to address the skewness bubble issue. However, the direct application of such a strategy in agentic reinforcement learning scenarios may precipitate severe off-policy challenges.
% %Simultaneously, the time-consuming nature of environment interactions is also a primary contributor to significant GPU underutilization. Table 1 shows average interaction end-to-end time of different environments. Though environments like code interpreter may occupy acceptable e2e latency, intricate external tool interactions, like search engine or even actions associated with VLA, introduce substantial, non-negligible interaction time, leaving GPU idle and causing great bubble, which we classify as a turn-level agentic bubble. To the best of our knowledge, this is the first work to define such kind of new type bubble in agentic RL training.

% %\textbf{How to scale up environments in a principled manner} serves as the other key challenge, stemming from the need to build a generalist agent that has the ability to handle diverse tasks, which is indeed the ultimate goal of RL. In \textit{multi-task} setting, agent needs to learn to interact with the most suitable environment, which naturally calls for a need for managing different environments. However, mainstream framework all treats environment as fixed and existing objects, where users are required to prepare the required environment, allocate resources in advance and incorporate hard code into the framework for invocation, which brings severe inflexibility. Meanwhile, for sandbox-type environment, each service is restricted with specific max concurrency and users typically need to perform horizontal scaling in order to fully utilize distributed resources, leading to poor scalability. To be worse, when some environment has trouble executing actions, the fixed logic of framework makes it impossible to migrate failed requests. Although some users are inclined to leverage third-party platforms for provisioning the necessary environments for tool invocation, such approaches, even those employing a serverless architecture, invariably incur substantial supplementary financial expenditures for the user.

% %These two challenges naturally give rise to a fundamental question: \textbf{whether a universal solution can be developed to abstract all environments and manage all resource allocation at a lower level, while dispatching all environmental interaction requests at a higher level?} This solution should also guide the filling of the corresponding "turn-level agentic bubble," analogous to how researchers have previously addressed the "common skewness bubble." 

% %Based on this, we propose AIO, a novel architecture conceptualized to function as a general and high-efficiency I/O layer that mediates agent-environment interactions. AIO is engineered for seamless integration into contemporary reinforcement learning frameworks with no effort, thereby effectuating a clear decoupling of the environmental interaction substrate from the core algorithmic architecture.

==> textFiles/6Implementation.tex <==
\section{Implementation}
\label{6}
 
\X is implemented in around 8k lines of Python code.

%\noindent\textbf{Batch Conductor.} Batch conductor is built upon the codebase of verl\cite{Sheng_2025} with commit id 1c1d53d. Since, during our development, verl had not supported sglang and multi-turn in fully async policy, we integrated such capabilities into our system with 1k LoC. Simultaneously, action-level abstraction and speculative partial rollout were implemented with around 1k LoC, establishing a highly efficient dataflow tailored for agentic RL training.

%\noindent\textbf{IO Layer.} IO Layer is implemented with 5.3k LoC. The Proxy serves as the centralized controller within the IO Layer, deployed as a service, exposing FastAPI endpoints, such as \emph{/get\_server} and \emph{/completion\_task} to RL framework. The Proxy maintains a resource\_pool to track the available environments and load status across different servers. Additionally, it incorporates a concurrency\_monitor to record actual concurrency bound and average tool interaction latencies over the preceding time step. These metrics serve as the critical basis for dynamic auto-scaling decisions. Resources on distributed servers are managed by the WorkerManager, which operates as a separate thread on each individual server. The underlying infrastructure abstracts the execution logic for different environments. Though our current implementation now only supports Code Interpreter and Local Retriever environment, IO Layer is architected to handle arbitrary complex environments, including VLA.

==> textFiles/8discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% Need to discussed bsz control here, like what concur does.

\noindent\textbf{Off-policy staleness.}
Previous works ~\cite{team2025kimi, fu2025areal} have proven that staleness thresholds can prevent gradient bias and maintains training stability.
\X uses \texttt{async\_factor} to strictly limits the staleness samples each step, thus preserving training convergence.
%\X follows the framework used by asynchronous RL. 
%Prior work~\cite{fu2025areal} shows this introduces no algorithmic loss: trajectories record their behavior policy, and the training objective corrects policy mismatch via the importance ratio, recovering the PPO-style objective.
%\X preserves this rule: trajectories are admitted only if they satisfy the staleness bound, maintaining algorithmic fidelity while improving throughput.

% \X follows the bounded-staleness setting used by asynchronous RL frameworks.
% Prior systems such as AReaL \cite{fu2025areal} show that this does not necessarily introduce algorithmic loss: each trajectory records the behavior policy \zmh{that generated it}, and the training objective can correct the policy mismatch through the importance ratio between the current policy and the behavior policy. 
% In expectation, this recovers the corresponding PPO-style objective, while bounding staleness keeps the ratio from drifting too far and avoids high-variance updates.
% \X does not modify this algorithmic rule. 
% Our scheduler only changes when a rollout request is executed to fill turn-level agentic bubbles; it does not change the action probabilities, reward computation, or advantage estimation. 
% Each trajectory is still tagged with its actor version and is admitted to training only if it satisfies the bounded-staleness constraint. 
% Therefore, \X preserves the same algorithmic fidelity as the underlying bounded-staleness RL framework, while improving throughput through scheduling.







==> textFiles/ex_abstract.tex <==
\section{Extended abstract}

Agentic Reinforcement Learning (RL) trains Large Language Models (LLMs) to solve complex tasks through iterative interaction with external environments. 
%Driven by this paradigm, LLMs have evolved from simple language assistants into agents that complete real-world software, web, and scientific workflows~\cite{guo2025deepseek, deepresearch2025, jin2025search, lu2025arpo, lu2025deepdive, feng2025group}.
% Agentic Reinforcement Learning (Agentic RL) has emerged as an important paradigm, enabling Large Language Models (LLMs) to solve complex tasks through iterative interaction with external environments. 
Driven by this paradigm, the applications of LLMs have evolved from simple language assistants into sophisticated agents capable of solving complex, real-world problems.
This paradigm also motivates the emergence of industry products such as Claude Code ~\cite{claudecode} and Deep Research ~\cite{deepresearch2025}.
%However, this emerging paradigm introduces two new systematic challenges that were previously overlooked.
%\zmh{However, this emerging paradigm introduces two unique system problems: \textit{how to schedule multi-turn rollouts to maximize end-to-end training throughput}, and \textit{how to manage the external environments in a scalable and cost-efficient manner}.}


%First, similar to traditional RL, agentic RL still suffers from pipeline bubbles arising from the sequential dependency between training and rollout, as well as skewness bubbles resulting from skewed distribution of response length within one batch.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{Figure/plot/rollout_scheduling.pdf}
%     % \vspace{-0.5\baselineskip}
%     %\caption[Caption for LOF]{(a) Trajectory-level scheduling, as used in modern agentic RL frameworks such as SLIME and VeRL. (b) Action-level scheduling, adopted in RollFlash, separates the GPU controller from the environment controller to saturate GPU utilization, but may compromise overall training throughput. (c) Priority-aware scheduling, which enables preemptive execution across samples.}
%     \caption[Caption for LOF]{Rollout scheduling policies. (a) Trajectory-level scheduling but introduces turn-level agentic bubbles. (b) Action-level scheduling, which saturates GPU but may even compromise training performance.}
%     \label{fig:rollout_scheduling}
%     \vspace{-1.5\baselineskip}
% \end{figure}
%A typical agentic RL training pipeline consists of three stages: \textit{rollout}, \textit{reward} and \textit{training}.
%During rollout, each prompt is replicated into multiple trajectories and each trajectory alters between model generation and environment interaction until reaching a terminal state.
%During reward, the quality of agent's action is evaluated by a scalar reward signal.
%During training, the agent LLM collects trajectories to update its weights and then synchronizes the updated weights to the rollout stage for the next iteration.
Similar to conventional single-turn RL, agentic RL training is dominated by the rollout stage, which accounts for over 70\% of total wall-clock time ~\cite{qin2025seer}.
%Existing systems have extensively optimized the training pipeline to mitigate pipeline bubbles arising from the sequential dependency between training and rollout and the straggler-induced skewness bubbles ~\cite{fu2025areal, gao2025rollpacker, qin2025seer}.
Existing RL systems mainly optimize this phase by mitigating straggler-induced skewness bubbles ~\cite{fu2025areal}.
%The skewness bubble issue is exacerbated in multi-turn settings due to uncertainty of turn numbers and imbalance interaction time.
%In such scenarios, generating a single trajectory requires frequent interactions with external environments, forcing GPU to stall until the completion of interaction.
%Beyond this shared characterization, the multi-turn nature of agentic trajectories introduces two unique system challenges: multi-turn rollout scheduling on the generation side and environment resource management on the interaction side.
Beyond this shared characterization, the multi-turn nature of agentic trajectories introduces unique system challenges: efficient rollout scheduling policy for maximizing end-to-end training throughput, and scalable environment interaction to backbone such flexible scheduling policy.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/plot/tidee.pdf}
    % \vspace{-0.5\baselineskip}
    %\caption[Caption for LOF]{(a) Trajectory-level scheduling, as used in modern agentic RL frameworks such as SLIME and VeRL. (b) Action-level scheduling, adopted in RollFlash, separates the GPU controller from the environment controller to saturate GPU utilization, but may compromise overall training throughput. (c) Priority-aware scheduling, which enables preemptive execution across samples.}
    \vspace{-0.5\baselineskip}
    \caption[Caption for LOF]{Existing work versus \X.}
    \label{fig:rollout_scheduling}
    \vspace{-1\baselineskip}
\end{figure}

%On the one hand, multi-turn paradigm introduces \textit{turn-level agentic bubbles}: trajectories stalled in external tool interaction may still occupy GPU generation slots.
First, for rollout scheduling, mainstream RL frameworks ~\cite{slime_github} typically adopt trajectory-level scheduling, where each trajectory is treated as an indivisible execution unit.
This coarse granularity ignores generation--interaction state transitions, thereby leaving GPU underutilization, which we call \textit{turn-level agentic bubbles}.
%As shown in Figure ~\ref{fig:rollout_scheduling}a, mainstream RL frameworks~\cite{slime_github, verl} adopt trajectory-level scheduling, treating each trajectory as an indivisible execution unit. 
%This policy is unaware of the transition between generation and tool interaction, allowing a trajectory to hold GPU generation slots while waiting for tool execution, which creates GPU underutilization that we call \textit{turn-level agentic bubbles} (Figure ~\ref{fig:utilization}).
%We define this as \emph{turn-level agentic bubbles}.
%While the evolution of RL frameworks from colocation-based architectures\cite{Sheng_2025, wang2025distflow, hu2025openrlhf} to disaggregated architectures\cite{fu2025areal, slime_github} has effectively mitigated standard pipeline and skewness bubbles, it fails to address the unique challenges posed by turn-level agentic bubbles.
%Although RollFlash\cite{lu2025iirollflash} offers a potential solution to this specific bottleneck, its reliance on sample-level overlap overlooks the temporal discrepancy between environmental interaction and reasoning, and their simplistic overlap strategy may even hinder the sequential generation of the primary trajectory.
%This not only degrades training efficiency but may also worsen off-policy issues.
Recent works address this problem by decoupling generation controllers from environment controllers, allowing  one trajectory's generation overlap with another's tool interaction ~\cite{cao2025skyrl, lu2025iirollflash}.
Though this action-level scheduling policy maximizes rollout GPUs throughput, it may not accelerate training process since the trainer only waits for enough completed trajectory groups to form the next training batch, while this policy scattered rollout progress across samples.
Moreover, KV Cache pressure and eviction is amplified by multi-turn execution.
A trajectory may first generate, suspend during tool execution, and later resume after its KV Cache has already been evicted by other active trajectories ~\cite{li2025continuum}.
This causes repeated recomputation overhead.
What's worse, the action-level scheduling, while effective for eliminating GPU idle time, increases the number of interleaved active trajectories and thereby aggravates this problem.
Both these two problems pose challenges for an optimized rollout scheduling policy.
%They allow one trajectory's generation overlap with another's tool interaction.
%In this paper, we refer to this design as \textit{action-level scheduling}: generation actions and environment-interaction actions are scheduled independently, allowing the generation of one trajectory to overlap with the tool interaction of another, as illustrated in Figure ~\ref{fig:rollout_scheduling}b.
%We refer to their design as action-level scheduling, as shown in Figure~\ref{fig:rollout_scheduling}b.
%This scheduling policy successfully maximizes rollout GPUs utilization.
%Nevertheless, GPU saturation alone is not equivalent to end-to-end training throughput.
%For the trainer, a rollout step completes only when enough complete sample groups are available to form the next training batch.
%Thus, the global rollout span is determined not by the aggregate number of generated tokens, but by the completion time of the sample groups that unblock training.
%A scheduler that maximizes local rollout throughput may still delay critical groups and leave the trainer waiting.
%Thus, the scheduling policy that only maximizes rollout throughput could even delay training due to scattered generation progress.
%While this policy improves rollout GPU utilization, the rollout throughput improvement may not translate into higher end-to-end training throughput. 
%The trainer can proceed only after enough complete sample groups are available for the next training batch. 
%Therefore, a scheduler that maximizes instantaneous rollout throughput may scatter progress across many groups and delay the completion of training-critical groups.

%Meanwhile, multi-turn execution further amplifies KVCache pressure.
%These observations raise a fundamental question: \textit{how should rollout scheduling be designed to accelerate end-to-end agentic RL training?}




Second, for scalable environment interaction, the challenge is not merely the safe execution and isolation of each tool sandboxes, but to sustain the high environment concurrency required by fine-grained rollout scheduling.
Action-level scheduling increases the number of active trajectories so that rollout GPUs can consume ready trajectories while others wait for tool execution. 
However, if the environment side cannot support this concurrency, generation workers are  blocked by interaction-side stalls, preventing action-level scheduling from fully realizing its benefit.
Thus, scalable environment interaction in fact places a strong demand on high-density sandbox deployment.
%For environment resource management, existing systems ~\cite{wang2025openhands, yang2024swe, dai2026cuda} typically run environment interactions inside isolated sandboxes, often implemented with microVMs ~\cite{agache2020firecracker, cloudhypervisor}.
%Second, agentic RL relies on external environments for tool interaction.
%To safely execute arbitrary tool actions, existing systems typically run environment interactions inside isolated sandboxes, often implemented with microVMs ~\cite{agache2020firecracker, cloudhypervisor}.
%This strong isolation is necessary for safety, but the conservative allocation mechanism significantly reduces deployment density.
%A sandbox is usually launched from a prebuilt image and configured with a fixed virtual memory limit.
%In production, the number of sandboxes placed on each node is often conservatively bounded by this maximum memory limit to avoid failures.
%However, as shown in Figure ~\ref{fig:online_sandbox_memory_usage}, the actual resident memory of a sandbox is frequently far below its configured upper bound, which is called "memory stranding" ~\cite{fuerst2022memoryharvesting,li2023pond,javadi2019scavenger}.
%Static placement therefore wastes substantial memory capacity.
%Moreover, treating sandboxes as fully independent instances ignores an important property of Agentic RL: many sandboxes are highly similar.
%Trajectories from the same sample group are often initialized from the same environment template, execute similar setup code, and share a large fraction of unchanged memory pages.
%Existing sandbox deployment mechanisms fail to exploit this structure, resulting in "state duplication" ~\cite{saxena2022memorydeduplication, huang2024trenv} across trajectories, \textcolor{blue}{where similar sandboxes hold redundant copies of identical pages.}
However, in production, sandboxes are conservatively packed by their configured memory ceilings, even though their actual resident set is far smaller, which leads to "memory stranding" ~\cite{fuerst2022memoryharvesting}. 
Worse yet, existing systems treat sandboxes as independent instances and overlook the structural property of agentic RL: a sample group consists of multiple rollouts sharing the same prompt. Therefore, trajectories within the same sample group are launched from identical templates and execute nearly identical setup code, so a fraction of their pages are byte-identical. 
This leads to "state duplication" ~\cite{saxena2022memorydeduplication} across sandboxes that could otherwise share memory.



Efficient agentic RL system therefore requires two complementary capabilities: an effective rollout scheduling policy that maximizes training throughput, and a scalable, cost-efficient environment manager that backbones such scheduling policy.
%\zmh{To address these challenges, we propose \X, a fully disaggregated system for Agentic RL training.}
To the end, we propose \X, a fully disaggregated system for agentic RL training, as shown in Figure ~\ref{fig:rollout_scheduling}.
\X decouples training, rollout generation, and environment interaction into independently managed components, and introduces two key mechanisms: a \textit{priority-aware action scheduler} for end-to-end training throughput, and an \textit{environment resource manager} for cost-efficient environment interaction.

The priority-aware action scheduler retains the benefits of action-level scheduling by separating generation workers from environment workers.
Additionally, as illustrated in Figure ~\ref{fig:rollout_scheduling}a, it incorporates priority into our scheduling decisions.
\X defines critical groups as unfinished groups whose completion is most likely to unblock the next trainer batch.
At runtime, \X uses length-prediction-based heuristics to identify such groups and prioritizes their execution.
To enforce this priority, \X co-designs the RL framework and rollout engine to provide priority-aware GPU-slot execution, ensuring that high-priority samples are scheduled ahead of others.
Beyond GPU scheduling, \X introduces priority-aware KV Cache residency.
It employs trajectory-aware radix cache and uses a three-tier KV Cache model for admission control and eviction decisions.
This design preserves KV Cache entries of high-priority trajectories on a best-effort basis.
Furthermore, \X performs priority-aware request orchestration to mitigate the imbalanced distribution of high-priority samples across rollout workers.
It monitors high-priority KV Cache pressure across rollout workers and migrates requests together with their reusable prefix cache to reduce KV contention of high-priority samples.

%The environment resource manager treats external environments as first-class cluster resources rather than task-private sandbox fleets.
The environment resource manager provides scalable interaction by page-grained and high-density sandbox deployment, with details shown in Figure ~\ref{fig:rollout_scheduling}b.
%The environment resource manager enables page-grained, high-density sandbox deployment.
%At cluster scope, \X uses a global controller to allocate sandboxes from a shared environment pool, enabling global admission control and avoiding uncoordinated overcommitment across concurrent agentic RL tasks.
At cluster scope, \X provides scalable interaction by a global controller to allocate sandboxes from a shared environment pool and hide deployment details to the framework.
At node scope, \X introduces page-level sandbox placement and dynamic admission control to maximize deployment density while preventing memory overcommitment.
To exploit similarity among agentic trajectories, \X further builds a group-level page sharing pool.
Trajectories from the same sample group share snapshot pages whenever possible: read-only pages are mapped to the same write-protected physical pages, and private copies are created lazily through copy-on-write upon modification.
This preserves sandbox isolation while substantially reducing redundant memory consumption.

We implemented \X in 24k lines of Python, Rust and Golang, and the code will be released upon publication.
We conduct extensive evaluations to validate the effectiveness of \X.
%Experimental data shows that \X outperforms state-of-the-art RL systems ~\cite{slime_github, lu2025iirollflash, kang2026thunderagent} and achieves 1.10$\times$--2.89$\times$ speedup. 
Experimental data shows that \X outperforms state-of-the-art RL systems, achieving 1.07--3.26$\times$ end-to-end training speedup over Slime ~\cite{slime_github}, 1.06-4.24$\times$ speedup over RollFlash ~\cite{lu2025iirollflash}, and up to 2.67$\times$ speedup compared to ThunderAgent ~\cite{kang2026thunderagent}.
Meanwhile, \X reduces environmental costs up to 89\% compared with E2B~\cite{e2bsandbox2024}, a representative and widely-use sandbox platform.

==> textFiles/name.tex <==
\begin{algorithm}[t!]
\caption{Event-Driven Preemptive Scheduling Workflow}
\label{alg:scheduling}
\begin{algorithmic}[1]
\footnotesize
\State \textbf{Global:} $Q_{list} \leftarrow [Q_{off}, Q_{prio\_can}, Q_{pot}, Q_{can}]$ 
\State \textbf{Global:} $Q_{pend}$ 
\State \textbf{Global:} $L_{active}, N_{gen}, Limit$

\Function{ScheduleLoop}{} 
    \While{True}
        \State $found\_task \leftarrow \textbf{false}$
        
        \For{$Q$ \textbf{in} $Q_{list}$}
            \State $req \leftarrow Q.front()$ 
            \If{$req \neq$ \textbf{null}}
                \If{\Call{IsHigh}{$req$}} 
                    \If{$N_{gen} \ge Limit$}
                        \State \Call{PreemptLast}{$L_{active}$} 
                    \EndIf
                    \State $Q.pop()$ 
                    \State \Call{RunStream}{$req$}
                    \State $found\_task \leftarrow \textbf{true}$
                    \State \textbf{break} 
                \Else 
                    \If{$N_{gen} < Limit$}
                        \State $Q.pop()$ 
                        \State \Call{RunStream}{$req$}
                        \State $found\_task \leftarrow \textbf{true}$
                        \State \textbf{break} 
                    \Else 
                        \State \Call{Wait}{$N_{gen}<Limit$ \textbf{or} $Q_{off}$.HasData}
                        \State $found\_task \leftarrow \textbf{true}$
                        \State \textbf{break} 
                    \EndIf
                \EndIf
            \EndIf
        \EndFor
        
        \If{$found\_task$} \textbf{continue} \EndIf
        
        \If{$N_{gen} \ge Limit$} 
            \State \Call{Wait}{$N_{gen} < Limit$ \textbf{or} $Q_{off}$.HasData}
            \State \textbf{continue}
        \EndIf
        
        \State $req \leftarrow Q_{pend}.pop()$
        \If{$req \neq$ \textbf{null}} \Call{RunStream}{$req$} \EndIf
    \EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{RunStream}
\label{alg:dispatch}
\begin{algorithmic}[1]
\small 
\Function{RunStream}{$req$} 
    \If{$st$ is \texttt{is\_cancel}} 
        \If{$req$.is\_Preemptive} 
            \Call{Push}{$Q_{\text{prio\_can}}, req$}
        \Else 
            \Call{Push}{$Q_{\text{can}}, req$} 
        \EndIf
    \ElsIf{$st$ is \texttt{is\_tool}} 
        \Call{Push}{$Q_{\text{bef\_int}}, req$}
    \ElsIf{$st$ is \texttt{is\_done}} 
        \Call{Push}{$Q_{\text{res}}, req$}
    \ElsIf{$st$ is \texttt{finish\_tool}} 
        \If{$req$.is\_high} 
            \Call{Push}{$Q_{\text{off}}, req$}
        \Else 
            \Call{Push}{$Q_{\text{pot}}, req$} 
        \EndIf
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}


\noindent\textbf{Limitations of the Other Disaggregation Works.}
%还有没有其他类似verl进行分离的工作
%先讲完全不解耦的工作，说出他们的问题
%为了解决吞吐量的问题，再说做了解耦生成和训练的工作，说出他们的问题
%之后再说将环境解耦的工作，rstar2-agent, verlTool（这两个的问题在Provisioning Trade-off中说的，他们用了静态资源分配）
To address the throughput bottlenecks, the architecture of RL training systems has evolved from integrated colocation to progressively finer-grained disaggregation. 
However, each stage retains structural limitations when applied to agentic RL.

Colocated architectures, such as HybridFlow~\cite{Sheng_2025} and Distflow~\cite{wang2025distflow}, focus on optimizing distributed training efficiency through programming abstractions or specialized colocated system designs.
While HybridFlow simplifies user invocation by abstracting the dataflow, its generation and training logic remain tightly coupled or compete for shared resources.
This lack of systemic decoupling forces generation tasks to pause during training phases to release resources, which significantly limits the overall training speed.

To resolve resource contention, systems like AREAL~\cite{fu2025areal}, SLIME~\cite{slime_github}, and AsyncFlow~\cite{han2025asyncflow} advance the field by physically decoupling rollout generation from training.
This separation allows dedicated workers to process asynchronous dataflows, often leveraging off-policy training settings to maximize throughput.
However, despite this architectural decoupling, these systems fail to optimize for the turn-level agentic bubbles inherent to agentic scenarios, leading to severe inefficiency.
As the agent learns to engage in complex tasks, the increasing number of interaction turns causes the GPU sources to remain locked during long I/O waits.
This prevents the scheduler from reassigning GPU resources to pending tasks, creating substantial turn-level bubbles.
Most recently, works like rStar2-Agent~\cite{shang2025rstar2} and VerlTool~\cite{jiang2025verltool} have begun to decouple environment execution from the LLM process to support complex tool use.
While they isolate the execution runtime, they typically treat environment resources as static entities managed by fixed pools.
As we discuss above, this static management fails to address the provisioning trade-off in dynamic agentic scenarios.
